Insurance design and arson-type risks

We design the insurance contract when the insurer faces arson-type risks. The optimal contract must be manipulation-proof. It is therefore continuous, it has a bounded slope, and it satisfies the no-sabotage condition when arson-type actions are free. Any contract that mixes a deductible, coinsurance and an upper limit is manipulation-proof. We also show that the ability to perform arson-type actions reduces the insured's welfare as less coverage is offered in equilibrium.

==> concluding_remarks.tex <==

%Though Bob likes his sledgehammer, we don't want him to use it on his bike.

We conclude with a few observations. First, notice that in proving Proposition 2
we never used the underlying probability 
properties except for the fact that the two
integrals in \eqref{Problem I} are finite. This means that we could have
considered different decision criterion. For instance, by replacing $\mathbb{P}$
with a capacity $\nu$ in one integral and integrating in the sense of Choquet
instead of Lebesgue. This would have changed nothing to the veracity of Proposition 2,
provided that the set of solutions to \eqref{Problem I} remains non-empty.\\

Which brings us to the two problems of existence and uniqueness. Existence was
implicitly guaranteed by the formal association with the problem of
\citet{spaeter1997design}. Uniqueness is not. While the
contracts found in lemma 4, fact 1 and lemma 5 are unique, we were unable to
prove uniqueness in the general case. The
difficulty comes from the observation that the cost $c$
must be recouped \textit{on average} and not state-by-state.
The problem remains open.\\

Finally, notice the following: (A) we worked by backward induction from the
last action taken in the game and (B) the class of contracts robust to
arson-type risks contains all contracts mixing co-insurance and deductible.
This means that there are no reasons to think \textit{a priori} that
complexifying the model would fundamentally change the
observations made in the text. In particular, enriching the model with notions
of ex-ante hidden action or information would most likely change nothing about
the fact that the optimal contract must be robust to arson-type risks.

==> introduction.tex <==

Suppose Bob was just involved in a bicycle accident. After the fact,
an officer of the law provided Bob with a certificate indicating that the automobile
driver was responsible for the accident. The certificate does not, however,
specify how bad the damage inflicted to Bob's steel steed was. Which types of
insurance contracts will incentivize Bob to take a sledgehammer to his bicycle before
taking a picture and filling his insurance claim?\\

\citet{huberman1983optimal} was first to point out that the possibility of
inflating an insurance claim by physically destroying an object imposes strong
structure on the type of contract which can be offered by an insurer.
They show that (completely) vanishing deductibles strongly incentivize the insured to
augment the damage. In their model, the next best contract is a simple
deductible\label{fig1:sub1}.\\

\citet{picard2000design} uses a similar argument to guarantee that his model's optimal
contract is continuous. The author also defines the risk
of destroying the object as an "arson-type" risk to distinguish it
from other ex-post risks of defrauding the contract\footnote{See Picard's
chapter in \citet{dionne2000handbook} for a review of the different notions of
fraud risks.}.\\
  
We use results from \citet{Lauzier2019positioningmaths} and
\citet{Lauzier2019securitydesign} to show that the arguments made in 
\citet{picard2000design} and \citet{huberman1983optimal} are two sides of
the same coin. We show that when there are arson-type risks the optimal contract
must be continuous and have a bounded slope. Ipso facto, any contract
mixing coinsurance and deductible will be robust to these risks.\\

After a brief literature review, we introduce and solve the model then conclude by
providing a few observations about our findings' robustness. 
\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
     \begin{tikzpicture}
        \draw[<->] (0,5) -- (0,0) -- (5,0);
        \draw[blue,thick](0,0) -- (2,0) -- (4,4); 
        \draw[gray,dotted] (0,0) -- (4,4);
        \node[below] at (5,0) {$X$};
        \node[left] at (0,5) {$Y$};
        \node[below] at (2,0) {$d$};
    \end{tikzpicture}  
    \caption{completely disappearing}
    \label{figure1:sub1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \begin{tikzpicture}
        \draw[<->] (0,5) -- (0,0) -- (5,0);
        \draw[blue,thick](0,0) -- (2,0) -- (4,2); 
        \draw[gray,dotted] (0,0) -- (4,4);
        \node[below] at (5,0) {$X$};
        \node[left] at (0,5) {$Y$};
        \node[below] at (2,0) {$d$};
    \end{tikzpicture}  
    \caption{simple}
    \label{figure1:sub2}
\end{subfigure}
\caption{deductibles}
\end{figure}

\subsection*{Literature review}

\citet{huberman1983optimal} contains the earliest mention of arson-type risks
which we are aware of.  The authors analyze the optimal
insurance contract when respecting the contract involves non-actuarial costs
such as administrative cost. Their model's optimal contract is a completely
disappearing deductible, and the authors observe that this type of contract is
infrequently observed in real life, if at all. They show that if the insured
can cause extra damage then their model's next best contract is a simple
deductible.\\

\citet{picard2000design}'s introduction of arson-type risks is similar to
\citet{huberman1983optimal}'s. \citet{picard2000design} designs the optimal
insurance contract when the insured can defraud the contract and manipulate
the audit costs. The model's optimal contract is discontinuous, another oddity
infrequently observed in real life. The author then shows that this
discontinuity disappears when there are arson-type risks.\\

Both the contract's continuity and its bounded slope obtain from the same mathematical
result. Formally, the manipulation stage of the game defines an optimisation
problem. As these contracts can be discontinuous as stated in \citet{picard2000design}
the first-order conditions cannot be used. This is where the results of \citet{Lauzier2019positioningmaths}
become necessary. These results also inform that the value function of the
manipulation stage's optimisation problem is continuous and has a bounded slope.\\

Using an argument similar to one made in \citet{Lauzier2019securitydesign} 
we determine that the shape of the contract is continuous and has a bounded slope.
This is because replacing a contract by the value function of the
optimisation problem it defines does not change the amount of insurance
provided. The new contract does not induce manipulation, it is
therefore cheaper as the expected waste due to manipulation is priced by the
insurer at nil.\\

While \citet{Lauzier2019securitydesign} obtained acceptable manipulations
we cannot phantom them in the case of insurance contracts. In insurance
contracts, the possibility of manipulations simply hurts the insured by
lowering the protection by the insurer in equilibrium. Since all contracts
mixing coinsurance and deductibles are robust to arson-type risks, there
does not seem to be a trade-off between the prevention of arson-type
manipulations and the provision of incentives to prevent ex-ante moral
hazard. This is exactly the opposite result as that obtained in 
\citet{Lauzier2019securitydesign}.\\

We will discuss \citet{spaeter1997design} in the main text and we refer to
\citet{dionne2000handbook} for an introduction to the Arrow-Borch-Raviv model.\\


==> model.tex <==

The three stage proof will structure the presentation. We start by showing 
that optimal contracts accounting for arson-type risks 
must be continuous and have a bounded sloped.
This implies that we can substitute our optimisation problem by a simpler one. This
new optimisation problem is formally almost identical to the one found in
\citet{spaeter1997design}, modulo an extra constraint which is not always
binding. The latter allows us to characterize many cases, though
the final derivations will be left to the reader.\\

\subsection*{Notation and problem}
We use standard notation throughout. Let $S$ be a set of states of the world
and let $\mathbb{P}$ be the probability of state $s\in S$. Let the function
$X:S \rightarrow [0,M]$ be a continuous random variable representing the risk
to be insured against, with $X$ having full support $[0,M]$ and some mass at
$0$, said mass representing the possibility that no accident ever occurs. 
Let the function $c:[0,M] \rightarrow \mathbb{R}_+$ be the cost of
respecting the insurance contract and let $Y:[0,M]\rightarrow [0,M]$ be the
state-contingent, variable part of the contract\footnote{ So $Y\in
B_+(\mathcal{B}([0,M]))$, the space of non-negative and bounded functions (sup-norm) which
are measurable with regard to the Borel $\sigma$-algebra of $[0,M]$.}. The
amount $H\geq 0$ denotes the price of the contract while $W_0>0$ is the initial
wealth of the insured and $\rho \geq 0 $ is the loading factor of the insurer.
As usual, the function $u:\mathbb{R}_+ \rightarrow \mathbb{R}_+ $ is a twice
differentiable and strictly concave Bernoulli utility function satisfying Inada
conditions.\\

\noindent The game proceeds as follows:

\begin{description}
    \item[Stage 1] the insured buys the insurance contract $Y$ at price $H$;
    \item[Stage 2] the state $s$ realizes and loss $X(s)$ occurs (Nature moves);
    \item[Stage 3] the insured observes the loss and decides to take hidden action
$z\in [0,M]$ to augment the damages;
    \item[Stage 4] the contract is implemented without renegotiation.
\end{description}

\noindent The solution concept is a weak Perfect Bayesian equilibrium where we assume
that the insured takes the insurer's most favoured action whenever indifferent\footnote{We refer to \citet{mas1995microeconomic} for a definition of our equilibrium concept.}.\\

By backward induction the optimal contract $(H,Y)$ solves the following
optimization program: {\scriptsize 
\begin{align}
    \sup_{H \geq 0, Y \in B_+(\mathcal{B}([0,M]))} & \int u(W_0 - H - X(s)- z(s) -g(z(s))+Y(X(s)+z(s)))d\mathbb{P} \tag{Problem I} \label{Problem I}\\
      s.t.\, & \,0 \leq Y \tag{LLI} \label{LLI}\\
      &\, Y \leq X \tag{BI} \label{BI}\\
           & \int Y(X(s)+z(s))+c(Y(X(s)+z(s))) d \mathbb{P} \leq (1+\rho)H \tag{PCI} \label{pci} \\
           & \forall s,\,  z(s) \in argmax_z \{ X(s) - z -g(z)+Y(X(s)+z)\} \tag{IIC} \label{iic}
\end{align}}
where \eqref{LLI} is the insured's limited liability constraint,
\eqref{BI} is the "boundedness constraint" stating that the insurer will never
pay more than the observed loss, \eqref{pci} is the insurer's participation constraint,
\eqref{iic} is the insured's interim incentive compatibility constraint
and the function
\begin{align*}
    g(z)= \begin{cases} +\infty &\text{ if } z<0\\ \beta z &\text{ if } z\geq 0 \end{cases}
\end{align*}
represents an extra cost of inflicting damage (Bob buying a sledgehammer).\\

 We now aim to prove that $Y$ is Lipschitz continuous with constant $\leq 1+\beta$.
\begin{assumption} We assume throughout that $Y$ is a non-decreasing function. \end{assumption}

The next statement is standard and will not be proved:
\begin{lemma} The insurer's participation constraint \eqref{pci} must be binding.\end{lemma}

The interim incentive compatibility constraint defines an optimisation
problem that was defined in \citet{Lauzier2019positioningmaths} as a
positioning choice problem. It immediately follows from Theorem 3 (p.12)
that the value function $V(s)$ is Lipschitz continuous with constant $\leq
1+\beta$. Paralleling the argumentation of Theorem 6 (p.19) in
\citet{Lauzier2019securitydesign} we conclude:

\begin{proposition} Any optimal contract $Y^*$ is manipulation-proof: for every $s \in S$ it is $0 \in argmax_z \{ X(s) - z -g(z)+Y(X(s)+z)\}$.\end{proposition}
\begin{proof} Suppose, by the way of contradiction, that $Y^*$ is optimal but
that there exists a $s\in S$ such that such that for every $z(s)\in argmax_z \{
X(s) - z -g(z)+Y(X(s)+z)\}$ it is $z(s)>0$. Consider the alternative contract
$(\Tilde{H},\Tilde{Y})$ for which we set $\Tilde{Y}(s)=V(s)$, where $V(s)$ is
the value function of the optimisation problem \eqref{iic} defined by $Y^*$.
Since $\Tilde{Y}(s)$ is Lipschitz with constant $1+\beta$ it is
manipulation-proof so $V(s)=\Tilde{V}(s)$, where $\Tilde{V}(s)$ is the value
function of the optimisation problem \eqref{iic} defined by $\Tilde{Y}$. In
words, this means that the insured receives state-by-state the same final
payoff under both contracts. By lemma 1, it holds that $\Tilde{H}<H$ and
$(\Tilde{H},\Tilde{Y})$ dominates $(H,Y^*)$, a contradiction.\end{proof}

We can intuitively understand proposition 2 as stating that arson-type risks
are fully priced by the insurer. The insured thus will prefer the cheapest contract
as he receives state-by-state the same final amount under both contracts.
Or, from Bob's perspective, he was offered two contracts offering the same protection.
An expensive
one which would allow him to take a sledgehammer to his bike and a cheaper one
which did not, so Bob, being a rational person, chose the cheaper option.\\

\begin{corollary} Any contract $Y$ must be Lipschitz and with slope $\leq 1+\beta$.\end{corollary}

Furthermore, together, corollary 3 and assumption 1 imply that, by
Theorem 3 of \citet{Lauzier2019positioningmaths}, the family of contracts
$$\{Y\in B_+(\mathcal{B}([0,M])):Y(s)=V(s)\}$$
consist of functions which are almost everywhere differentiable and
everywhere directionnally differentiable.\\

We can thus rewrite \eqref{Problem I} as
\begin{align}
    \max_{H \geq 0, Y \in B_+(\mathcal{B}([0,M]))} & \int u(W_0 - H - X(s) +Y(X(s))d\mathbb{P} \tag{Problem S} \label{Problem S}\\
      s.t.\, & \,0 \leq Y \leq X \label{S1}\\
            & slope(Y)\leq 1+ \beta \label{S2}\\
           & \int Y(X(s))+c(Y(X(s))) d \mathbb{P} = (1+\rho)H \label{S3}
\end{align}
under the implicit assumption that $Y\in C^0[0,M]$ \footnote{The space of
continuous functions on the close interval $[0,M]$.} is almost everywhere
differentiable and everywhere directionnally differentiable. Notice how
this problem, as rewritten, is almost identical to the problem studied in
\citet{spaeter1997design} except for the extra constraint $slope(Y)\leq 1+\beta$.\\

A deduction from the author's work informs when the constraint is binding.
While the constraint is not binding the authors' solution is also a
solution to \ref{Problem S}.
While the constraint is binding we must resolve \ref{Problem S}.

\begin{lemma}
If $c=0$ then the optimal contract entails full insurance, i.e. $Y=X$.
\end{lemma}

\begin{proof} Observe that for $Y=X$ constraint \eqref{S2} is never binding and
    for $c=0$ constraint \eqref{S3} collapses to
    $$ \int Y(X(s)) d \mathbb{P} = (1+\rho)H$$
    so problem \eqref{Problem S} is the standard Arrow-Borch-Raviv problem.
\end{proof}

This lemma tells us that \eqref{Problem S} becomes interesting only when $c>0$ somewhere.
This is because when $c=0$ Bob is completely insured this precludes any incentive
to take a sledgehammer to his bike.
\\

\begin{fact} If $Y^*$ solves the reduced problem
\begin{align}
\max_{H \geq 0, Y \in B_+(\mathcal{B}([0,M]))} & \int u(W_0 - H - X(s) +Y(X(s))d\mathbb{P} \tag{Reduced problem} \label{reduced problem}\\
  s.t.\, & \,0 \leq Y \leq X \nonumber \\
       & \int Y(X(s))+c(Y(X(s))) d \mathbb{P} = (1+\rho)H  \nonumber
\end{align}
of \citet{spaeter1997design} and $Y^*$ satisfies constraint \eqref{S2}
then $Y^*$ solves \eqref{Problem S}.
\end{fact}

This fact informs us that the only problematic case which must be handled is when the
contract $Y^*$ found in \citet{spaeter1997design} does not satisfy constraint
\eqref{S2} somewhere. Intuitively it seems natural to attempt fattening $Y^*$ sufficiently to 
satisfy $slope(Y)\leq 1+\beta$ thus solving \ref{Problem S}. This approach is sometimes fruitful but does not work in certain cases as we explain later. While intermediate cases will be left to the
reader we will characterise a simple case when $\beta=0$.

\begin{lemma}
If $\beta=0$, $Y_R^*$ solves \eqref{reduced problem} and $Y_R^*$ is a
  completely disappearing deductible then the unique solution $Y_I^*$ to
  problem \eqref{Problem I} is a simple deductible, i.e. a function of the form
$$Y^*_I(s)=\max\{0,X(s)-d\}$$ for $d\geq 0$.
\end{lemma}
\begin{proof}
    If $Y_R^*$ is a completely disappearing deductible then there exists a
    $\Tilde{s}\in S$ such that for every $X(s)\geq X(\Tilde{s})$ it is
    $Y_R^*(s)=X(s)$. This implies that there is a state $\Tilde{\Tilde{s}}\in S$
    such that for every $X(\overline{s})\geq X(\Tilde{\Tilde{s}})$ the constraint
    \eqref{S2} of problem \eqref{Problem S} will be binding and so $slope(Y_I^*(s))=1$
    on the set $[X(\Tilde{\Tilde{s}}), M]$. It is easy to check
    that\footnote{Either by "Guessing \& Verifying" in \eqref{Problem S} or working
    by contradiction assuming $Y_I^*(s)$ is increasing somewhere on
    $[0,X(\Tilde{\Tilde{s}}))$.}
    $slope(Y_I^*(s)) = 0$ on $[0,X(\Tilde{\Tilde{s}}))$.
    Setting $d=X(\Tilde{\Tilde{s}})$ we obtain that
    $Y^*_I$ can be written as $Y^*_I(s)=\max\{0,X(s)-d\}$.
\end{proof}

The possibility that people have to take a sledgehammer to their bicycles is 
priced into insurance contracts is the reason why Bob will never be offered
a completely disappearing deductible contract. Simply, though Bob would honestly
like to purchase such contract, he cannot. This is because no Bob
can commit to being honest.\\

The intuition that the contract solving problem \eqref{Problem S} is
simply a "flattening" of the solution to \eqref{reduced problem} is misleading.
By additivity of the Lebesgue integral, the insurer's participation constraint
states that the insurer should recoup the cost \textit{on average} and
\textit{not state-by-state}. This, fortunately, gives us some leeway in solving
\eqref{Problem S}. However, this also means that there are some cases
where we have to roll-up our sleeves and directly attack the problem.


